Incremental Maintenance of Maximal Cliques in a Dynamic Graph

We consider the maintenance of the set of all maximal cliques in a dynamic graph that is changing through the addition or deletion of edges. We present nearly tight bounds on the magnitude of change in the set of maximal cliques, as well as the first change-sensitive algorithms for clique maintenance, whose runtime is proportional to the magnitude of the change in the set of maximal cliques. We present experimental results showing these algorithms are efficient in practice and are faster than prior work by two to three orders of magnitude.

==> intro-bak.tex <==
%----------------------
\section{Introduction}
\label{sec:intro}
%----------------------

Graphs are widely used in modeling linked data, and there has been tremendous interest in efficient methods for finding patterns in graphs, an area often called ``graph mining''. A fundamental task in graph mining is the identification of dense subgraphs, which are groups of vertices that are tightly interconnected. 

Many big data applications need to identify dense subgraphs from an evolving graph that is changing with time as new edges are added and old edges are deleted. For example~\cite{AKS+13} were able to identify breaking stories from the Twitter message stream in real-time through mining dense subgraphs from an evolving graph. Analysis of communities within microblogging platforms~\cite{JS+07} can be performed through identifying dense structures within an evolving graph representing connections between users. Identifying dense substructures in a graph is a critical component of other mining tasks, such as identifying groups of closely linked people in a social network~\cite{hanneman-socialnw,LSZL2011,LSH2008}, identifying web communities~\cite{GKT05,KRRT1999,RH2005}, and in constructing the Phylogenetic Tree of Life~\cite{DABMMS2004,SDREL2003,YBE2005}.

Most current methods for identifying dense subgraphs are batch methods designed for static graphs. When presented with a graph $G$, they can enumerate the set of all dense subgraphs within $G$. Suppose we used such a batch method to identify dense subgraphs within a graph $G$; if $G$ changes slightly, say, by the addition of a few edges to yield $G'$, it is now necessary to enumerate all subgraphs within $G'$ all over again, even though the set of dense subgraphs may have only changed slightly in going from $G$ to $G'$. This is a source of serious inefficiency, so that methods designed for static graphs are not applicable to a graph that is changing frequently, and different methods are needed for handling a dynamic graph. From a foundational perspective, identifying dense structures in a graph has been a problem of long-standing interest in computer science, but even basic questions remain unanswered on dynamic graphs.

A dynamic graph evolves over time due to addition or deletion of edges and vertices. An example is a graph that represents an online social network where vertices represent people, and there is an edge between two vertices if the corresponding people are connected in the social network. Such a graph is continuously evolving through the addition and deletion of edges, as new connections are added and deleted. Such dynamic networks are common in areas such as transportation networks, telecommunication networks, transaction networks, etc. This work focuses on detection emerging dense subgraphs (a subgraph where vertices are tightly interconnected) in real time as the graph evolves over time. 

We are motivated by many applications where maintenance of maximal cliques in a dynamic graph is an important task. Chateau et al.~\cite{CRR11} proposed incremental techniques for the maintenance of approximate common intervals among genomes through the maintenance of maximal cliques in an appropriately defined dynamic graph. Hussain et al.~\cite{HM+15} proposed techniques for the maximum range-sum query over moving data through the maintenance of maximal cliques in an appropriately defined dynamic graph. Duan et al.~\cite{DL+12} propose incremental $k$-clique clustering algorithm where maximal clique maintenance is an important task. 


We consider the problem of maximal clique maintenance in dynamic graph when the graph evolves over time due to the addition of edges. A maximal clique is perhaps the most fundamental and widely studied dense subgraph. A clique $c$ in a graph $G$ is an induced subgraph where every pair of vertices of $c$ is connected. $c$ is a maximal clique if it is not a subgraph of another clique.  The algorithms proposed in the literature~\cite{S04, OV10, XC+14, SW+17} for clique maintenance are not efficient in the sense that  some of the works require to access existing maximal cliques that remain unaffected when the graph changes~\cite{S04, SW+17} and other works~\cite{OV10, XC+14} does not provide any theoretical dependence of the number of changes in the set of maximal cliques in the time complexity of enumerating the changes in the event of graph update.

Therefore, we need an efficient algorithm for the maintenance of maximal cliques such that we can enumerate the changes in the maximal cliques without accessing the existing maximal cliques that remain unaffected due to the change in the graph. Also, the computation time should be proportional to the size of the change in the set of maximal cliques, which means, the algorithm takes large amount of time when the size of change is large and takes small amount of time when the size of change is small. For example, consider an empty graph on $10$ vertices (no edges) and the graph becomes complete due to addition of a set of all possible edges. In this case, the size of change is small, because, only one new maximal clique will be formed which is a clique of $10$ vertices when the graph is updated. Consider another example where the initial graph with $10$ vertices where the vertices forms $5$ pairs and there exists edges from a vertex to all other vertices not in that pair. Clearly, the number of maximal cliques in this graph is $2^5$. Now when a new edge is added that connects two vertices in the same pair, observe that, each of these $2^5$ maximal cliques in the graph no longer remain maximal and $2^4$ new maximal cliques are formed in the updated graph. This shows an instance where the changes in the maximal clique can be larger than the number of maximal cliques in the original graph when only a single edge is added. Thus, an efficient algorithm be such that it will take less amount of time when the change is small and it will take large amount of time when the change is large. 


A dynamic graph algorithm is called {\em incremental} when only the addition of edges is considered and is called {\em decremental} when only the deletion of edges is considered. For example, a parallel algorithm due to Simsiri et al.~\cite{ST+16} maintains the connected components when the new edges are added. An algorithm due to Thorup~\cite{T99} do the same when the edges are deleted from the graph. When a dynamic graph algorithm can simultaneously handle addition and deletion of edges, it is called {\em fully dynamic} graph algorithm. An algorithm due to Wulff-Nilsen~\cite{W13} solves the fully dynamic graph connectivity problem. 

In this work we propose an efficient incremental algorithm for the maintenance of maximal cliques. Let $G = (V,E)$ be an undirected unweighted graph on vertex set $V$ and edge set $E$. A clique in $G$ is a set of vertices $C \subseteq V$ such that any two vertices in $C$ are connected to each other in $G$. A clique is called maximal if it is not a proper subset of any other clique.  Let $\cliques(G)$ denote the set of maximal cliques in $G$.

Suppose that we started from a graph $G = (V, E)$ and the state of the graph changed to $G' = (V, E \cup H)$ through an addition of a set of new edges $H$ to the set of edges in the graph $G$. See Figure~\ref{fig:init} for an example.
Let $\Lambda^{new}(G,G') = \cliques(G') \setminus \cliques(G)$ denote the set of maximal cliques that were newly formed in going from $G$ to $G'$, and $\Lambda^{del}(G,G') = \cliques(G) \setminus \cliques(G')$ denote the set of cliques that were maximal in $G$ but are no longer maximal in $G'$. Let $\Lambda(G,G') = \Lambda^{new}(G,G') \cup \Lambda^{del}(G,G')$ denote the symmetric difference of $\cliques(G)$ and $\cliques(G')$.
We ask the following question:


%for arxiv
%-------------------------------------------------------------------------------------
\begin{figure*}
\centering
\begin{tabular}{c}
	%\hspace{-2mm}
	\includegraphics[width=.5\textwidth]{pic1.png}\\
\end{tabular}
\caption{\textbf{Change in maximal cliques due to addition of edges. \textbf{$G$}: Initial graph; \textbf{$G'$}: Graph after adding edges $(3,5)$ and $(4,5)$ to $G$; \textbf{$G''$}: Graph after adding edges $(1,3)$ and $(1,4)$ to $G'$.}}
\label{fig:init}
%fig7
\end{figure*}
%-------------------------------------------------------------------------------------
%------------------------------------------------------------------------------
%\def\beforeCap{-0.2mm}
%\begin{figure*}
%  \def\width{0.2}
%  \def\widthI{0.8}
%  \centering
%  \hfill
%  \begin{subfigure}[t]{\width\textwidth}
%    \centering
%    \includegraphics[width = \widthI\textwidth]{pic1.png}
%    \vspace*{\beforeCap}
%    \caption*{Change in maximal cliques due to addition of edges. $G_1$: Initial graph; $G_2$: Graph after adding edges $(3,5)$ and $(4,5)$ to $G_1$; $G_3$: Graph after adding edges $(1,3)$ and $(1,4)$ to $G_2$.}
%  \end{subfigure}
%  \hfill
%  \begin{subfigure}[t]{\width\textwidth}
%    \centering
%    \includegraphics[width = \widthI\textwidth]{pic2.png}
%    \vspace*{\beforeCap}
%    \caption{Graph $G_n$ is formed from $H_n$ by adding four edges to
%    $S_0$.}
%  \end{subfigure}
%  \hspace*{\fill}
%  \caption{For the case $(n \mod 3) = 1$, $H_n$ and $G_n$ are non-isomorphic graphs on $n$ vertices, with $f(n)$ maximal cliques each, showing a counterexample to Theorem 2 of Moon and Moser~\protect\cite{MM65}}
%    \label{fig:intro}
%  \end{figure*}


%------------------------------------------------------------------------------


\begin{itemize}
%\itemsep0em 
%\item How large can the size of $\Lambda(G_1,G_2)$ be, especially for the cases when a small number of edges are added to $G_1$? To systematically study the problem of maintaining maximal cliques in a dynamic graph, we first need to understand what is the possible magnitude of change in the set of maximal cliques.

\item \modified{How large can the size of $\Lambda(G,G')$ be? To systematically study the problem of maintaining maximal cliques in a dynamic graph, we first need to understand the magnitude of change in the set of maximal cliques.}
\item How can we efficiently compute $\Lambda(G,G')$? Can we compute $\Lambda(G,G')$ quickly in cases when $|\Lambda(G,G')|$ is itself small? In other words, can we have {\em change-sensitive} algorithms for computing $\Lambda(G,G')$, whose time complexity is proportional to the size of $\Lambda(G,G')$? 
\item What is the performance of such algorithms in practice? In other words, how the algorithm performs in maintaining the changes in the maximal cliques in large graphs?
\end{itemize}

%--------------------------------
\subsection{Contributions}
%--------------------------------
We present progress towards answering the questions posed above. 

\modified{
\textbf{Magnitude of Change in the Set of Maximal Cliques:} Let $f(n)$ denote the maximum number of maximal cliques in a graph on $n$ vertices. A result of Moon and Moser~\cite{MM65} shows that $f(n)$ is approximately $3^{n/3}$. 

When a set of edges $H$ is added to graph $G = (V,E)$ resulting in graph $G' = (V,E \cup H)$, we present nearly tight upper and lower bounds for the maximum size of $\Lambda(G,G')$, taken across all possible graphs $G$ and edges $H$. We show that by the addition of a small number of edges to the graph $G$ on $n$ vertices, it is possible to cause a change of nearly $2f(n) \approx 2 \cdot 3^{n/3}$, which is a trivial upper bound on the magnitude of $\Lambda(G,G')$. Details are in Theorem~\ref{thm:lambdan}.

We encountered an error in the 50-year old result of Moon and Moser~\cite{MM65} on the number of maximal cliques in a graph, which is directly relevant to our bounds on the change in the set of maximal cliques. We present our correction to their result in Observation~\ref{obs:mm}.
}

\textbf{Maximal Clique Maintenance Algorithm:} We present incremental algorithm for maintaining the set of maximal cliques of a dynamic graph when the graph $G$ changes to $G'$ due to the addition of a batch of edges. We maintain the set of maximal cliques through separately maintaining $\Lambda^{new}(G,G')$: the set of new maximal cliques and $\Lambda^{del}(G,G')$: the set of subsumed maximal cliques. Thus, our maintenance algorithm consists of two parts: (1) Algorithm $\csnew$ for maintaining the set of new maximal cliques that uses maximal clique enumeration algorithm from static graph as a subroutine and (2) Algorithm $\cssub$ for maintaining the set of subsumed maximal cliques. The time complexity of $\csnew$ is $\mbox{$O(\Delta^3 \rho |\Lambda^{new}(G,G')|)$}$ where $\Delta$ is the maximum degree of the updated graph $G'$ and $\rho$ is the number of new edges in $H$ and the time complexity of $\cssub$ is $O(2^{\rho} |\Lambda^{new}(G,G')|)$. When $\rho$ is fixed, the time complexity of the maintenance algorithm is thus $\mbox{$O(\Delta^3 |\Lambda^{new}(G,G')|)$}$ which is linear in the number of new maximal cliques times polynomial in the maximum degree of the graph. When $\rho$ is set to $3\log_2\Delta'$ where $\Delta'$ is the maximum degree of $G$, the time complexity of the maintenance algorithm becomes $O(\Delta^3\log_2\Delta|\Lambda^{new}(G,G')|)$. To the best of our knowledge, our algorithm is the first change-sensitive algorithm for maintaining the changes in the set of maximal cliques when $\rho$ is constant or in the logarithmic order of the maximum degree of the original graph.

We also develop $\csnewttt$ for enumerating new maximal cliques, a practical variant of theoretically efficient algorithm $\csnew$, that uses worst case optimal and practically most efficient algorithm $\tomita$ due to Tomita et al.~\cite{TTT06} for maximal clique enumeration from static graph as subroutine and some technique for avoiding duplicate new maximal clique generation. We name our maintenance algorithm as $\sdiff$ that uses $\csnewttt$ for maintaining new maximal cliques and $\cssub$ for maintaining subsumed maximal cliques.

Our methods can extend to the decremental case, where the goal is to enumerate the change in the set of maximal cliques due to deletion of edges from the graph. Our methods can also be applied to the general dynamic case, where edges are both added to and removed from the graph. However, the fully dynamic case is not proven to be change-sensitive as discussed in Section~\ref{sec:dec}.



\textbf{Experimental Evaluation:} We present empirical evaluation of our algorithm using real world dynamic graphs as well as synthetic graphs. Our experimental study shows that $\sdiff$ can enumerate change in maximal cliques in a large graph with of the order of a hundred thousand vertices and millions of edges within a few seconds. We also compare $\sdiff$ with prior works and it turns out that our work significantly outperform prior solutions, including ones due to Stix~\cite{S04}, Ottosen and Vomlel~\cite{OV10}, and Sun et al.~\cite{SW+17}. For example, on the {\tt flickr-growth} graph, our algorithms are faster than~\cite{S04, OV10, SW+17} by a factor of more than a thousand. Noticeably, on the {\tt flickr-growth} graph, starting with an empty graph $\sdiff$ took around $40$ ms. overall to insert around $250$ batches incrementally (one batch at a time) each of size $100$ and maintain the changes, whereas prior techniques took $5$ min. to more than $2$ hours for computing the same.  More details are in Section~\ref{sec:expts}.

\remove{
\paragraph*{Enumerating the Change in the Set of Maximal Cliques:}
Let $G'=(V,E\cup H)$ denote the graph after adding edges $H$ to $G$. 

\textbf{(1)}~We present algorithms that take as input $G$ and $H$, and enumerate the elements of $\Lambda(G,G')$ in time proportional to the size of $\Lambda(G,G')$, i.e. the magnitude of the change in the set of maximal cliques. We refer to such algorithms as {\em change-sensitive} algorithms. To our knowledge, these are the first provably change-sensitive algorithms for maintaining the set of maximal cliques in a dynamic graph. 

The time taken for enumerating newly formed cliques 
 $\Lambda^{new}(G,G')$ is $\mbox{$O(\Delta^3 \rho |\Lambda^{new}(G,G')|)$}$ where $\Delta$ is the maximum degree of a vertex in $G'$ and $\rho$ is the number of edges in $H$. The time taken for enumerating subsumed cliques $\Lambda^{del}(G,G')$ is $O(2^{\rho} |\Lambda^{new}(G,G')|)$. \modified{Note that, when $\rho$ is constant, the time complexity of our algorithm is $O(\Delta^3|\Lambda^{new}(G,G')|)$ that is linear in the size of change times a factor ($\Delta^3$) related to the size of the graph. To the best of our knowledge, these are the first change-sensitive algorithm for the maintenance of maximal cliques in a dynamic graph. Also by setting the $\rho = 3\log_2\Delta'$ where $\Delta'$ is the maximum degree of $G$, the overall time complexity of our algorithm is $O(\Delta^3\log_2\Delta|\Lambda^{new}(G,G')|)$. Although the complexity with fixed size $\rho$ is better than variable size $\rho$ in terms of big-Oh notation, for the fixed size case, the high value of $\rho$ results in a high constant factor and that might have high impact in overall computation time.}

\textbf{(2)}~\modified{Based on our theoretically-efficient change-sensitive algorithms, we present practical algorithms for enumerating new and subsumed cliques and implementations of these algorithms. Our experimental study shows that they can enumerate change in maximal cliques in a large graph with of the order of a hundred thousand vertices and millions of edges. These significantly outperform prior solutions, including ones due to Stix~\cite{S04}, Ottosen and Vomlel~\cite{OV10}, and Sun et al.~\cite{SW+17}. For example, on the {\tt flickr-growth} graph, our algorithms are faster than~\cite{S04, OV10, SW+17} by a factor of more than a thousand}.

\textbf{(3)}~Our methods extend to the decremental case (\modified{through a reduction to the incremental algorithm}), where the goal is to enumerate the change in the set of maximal cliques due to deletion of edges from the graph. Our methods can also be applied to the general dynamic case, where edges are both added to and removed from the graph. \modified{However, the fully dynamic case is not proven to be change-sensitive as discussed in Section~\ref{sec:dec}.}
}
%{\color{red} Also say this works for decremental case.}
\remove{
%--------------------------------------------
\subsection{Relation to Prior Work}
%--------------------------------------------
}

%--------------------------------------------
\subsection{Related Work}
\label{ref:related}
%--------------------------------------------

{\bf Maximal Clique Enumeration in a Static Graph.} There is substantial prior work on enumerating maximal cliques in a static graph, starting from the algorithm based on depth-first-search due to Bron and Kerbosch~\cite{BK73}. A significant improvement to~\cite{BK73} is presented in Tomita et al.~\cite{TTT06}, leading to worst-case optimal time complexity $O(3^{n/3})$ for an $n$ vertex graph~\cite{MM65}. Other work on refinements of~\cite{TTT06,BK73} include~\cite{Koch01}, who presents several strategies for pivot selection to enhance the algorithm in~\cite{BK73}, and a fixed parameter tractable algorithm parameterized by the graph degeneracy~\cite{ELS10,ES11}.

There is a class of algorithms for enumerating structures (such as maximal cliques) in a static graph whose time complexity is proportional to the size of the output -- such algorithms are called \remove{``output-efficient"}``output-sensitive" algorithms. Many \remove{output-efficient}output-sensitive structure enumeration algorithms for static graphs, including~\cite{TI+77,CN85,MU04}, can be seen as instances of a general technique called ``reverse search''~\cite{AF93}. The current best bound on the time complexity of \remove{output-efficient}output-sensitive maximal clique enumeration on a dense graph $G=(V,E)$ is due to~\cite{MU04} which runs with $O(M(n))$ time delay (the interval between outputting two maximal cliques), where $M(n)$ is the time complexity for multiplying two $n\times n$ matrix, which is $O(n^{2.376})$. Further work in this direction includes~\cite{KW+01} and~\cite{JYP88}, who consider the enumeration of maximal independent sets in lexicographic order and~\cite{CK+11}, who consider the external memory model. Extensions to parallel frameworks such as MapReduce or MPI are presented in~\cite{SMT14,MT14}.




{\bf Maximal Clique Enumeration in a Dynamic Graph.}
In~\cite{S04,XC+14}, the authors present algorithms for tracking new and subsumed maximal cliques in a dynamic graph when a single edge is added to the graph. These algorithms are not proved to be change-sensitive, even for a single edge. In~\cite{S04}, the algorithm for enumerating new maximal cliques needs to consider (and filter out) maximal cliques in the original graph that remain unaffected due to addition of new edge. This can be wasteful, in terms of update time. \remove{the algorithm needs to store the set of all maximal cliques of the original graph, which is wasteful in terms of space. if a batch of many edges $H$ is added to a graph, an algorithm that recomputes the change in maximal cliques after each edge addition maybe very inefficient -- the change after the addition of all edges in the batch maybe very small, but the cumulative changes in maximal cliques during intermediate stages may sum up to a very large number.} Hence, such an algorithm cannot be change-sensitive. For example, consider the case of a graph growing from an empty graph on $10$ vertices to a clique on $10$ vertices. Only one new maximal clique has been formed by this batch, but numerous maximal cliques arise during intermediate steps -- if all these are enumerated, then the time complexity of enumeration is inherently large, even though the magnitude of change is small.

Ottosen and Vomlel~\cite{OV10} present an approach to enumerating the change that is based on running a maximal clique enumeration algorithm on a smaller graph, localized to the change in the set of edges and their algorithm supports addition of a set of edges. In contrast with our work, there are no provable performance bounds for this algorithm. Another difference is that the algorithm of~\cite{OV10} may not maintain the exact change in the set of maximal cliques, in certain cases, while our algorithms can maintain the change in the set of maximal cliques exactly.

Recently, Sun et al.~\cite{SW+17} present an algorithm for the same problem where they iterate over the set of maximal cliques of the original graph to derive the set of maximal cliques of the updated graph. Their algorithm is inefficient because they require to iterate over the entire maximal clique for maintaining the change in the set of maximal cliques which incurs many wasteful iterations when most of the maximal cliques remain unaffected.
 
%Prior works have not considered bounds on the magnitude of change that can be caused due to the addition (or deletion) of edges to the graph, and we are the first to do so.


{\bf Maintaining Other Structures on a Dynamic Graph.}
Other works on maintaining dense structures on a dynamic graph include \modified{maintenance of maximal bicliques in a dynamic bipartite graph~\cite{DT+17}}, maintenance of $k$-cores~\cite{SG+13,LYM14} and $k$-truss communities~\cite{HC+14}, and works on maintaining the densest subgraph on a dynamic graph~\cite{BKV12,MT+15}. \modified{Bicliques are the complete structures in bipartite graphs. The other structures: $k$-core, $k$-truss, and densest subgraph, are different from maximal cliques and maximal blcliques in that they do not require complete connectivity among different vertices within the structure}.

\remove{
{\color{red} Can you please make this paragraph more precise. It does not convey much information, and is hard to understand. Also, make sure that all the citations that were mentioned by the reviewers have been included.}
}
Some other recent work on query processing on large dynamic graphs includes~\cite{LB+15}, which proposes parallel and dynamic methods for queries such as average vertex degree, clustering coefficient distribution, distribution of shortest path distances, distribution of sizes of connected components, etc. In~\cite{KD13}, the authors present a data structure for executing snapshot retrieval queries on historical data. In~\cite{RL+11}, the authors propose a framework for processing queries such as shortest paths on historical evolving graph sequences. These works are related to maintaining structures on dynamic graphs, but are not related to enumerating dense structures.

\remove{   
\modified{In addition to structure enumeration in dynamic graphs, there have been some recent works~\cite{RL+11, KD13} on efficiently maintaining dynamic graphs in such a way that, we can efficiently answer the query to the dynamic graphs. {\color{red} what queries?} In~\cite{LB+15}, the authors addressed scalability and efficiency in terms of storage of dynamically evolving graphs by taking advantages of the commonalities of the graph at different time points of the evolution. {\color{red} again, for what queries?} However, the techniques are not related to our work because, none of these works discuss about dense structure enumeration problem.}
}

\remove{
%------------------------------
\subsection{Related Work}
\label{sec:related}
%------------------------------
There is substantial prior work on enumerating maximal cliques in a graph starting from the algorithm based on depth-first-search due to Bron and Kerbosch~\cite{BK73}. A significant improvement to~\cite{BK73} is presented in Tomita et al.~\cite{TTT06} using the idea of ``pivoting'', leading to a precise upper bound on the worst-case time complexity, showing worst-case optimality~\cite{MM65}. Other work on refinements of~\cite{TTT06,BK73} include~\cite{Koch01}, who presents several strategies for pivot selection to enhance the algorithm in~\cite{BK73}, and a fixed parameter tractable algorithm parameterized by the graph degeneracy~\cite{ELS10,ES11}.

Many output-efficient structure enumeration algorithms for static graphs, including~\cite{TI+77,CN85,MU04}, can be seen as instances of a general technique called ``reverse search''~\cite{AF93}. The current best bound on the time complexity of clique enumeration on a dense graph $G=(V,E)$ is due to~\cite{MU04} {\color{blue} which runs with $O(M(n))$ time delay, where $M(n)$ is the time complexity for multiplying two $n\times n$ matrix, which is $O(n^{2.376})$} \st{and is based on matrix multiplication}. Further work in this direction includes~\cite{KW+01} and~\cite{JYP88}, who consider the enumeration of maximal independent sets in lexicographic order and~\cite{CK+11}, who consider the external memory model. Extensions to parallel frameworks such as MapReduce or MPI are presented in~\cite{SMT14,MT14}. None of these consider the dynamic case.

There has been recent work on enumerating structures other than maximal cliques on dynamic graphs, including maintenance of k-cores~\cite{SG+13,LYM14}, and k-truss communities~\cite{HC+14}. External memory algorithms for maximal clique enumeration has been considered in~\cite{CK+11}. 

{\color{blue}In addition to structure enumeration in dynamic graphs, there have been some recent works~\cite{RL+11, KD13} on efficiently maintaining dynamic graphs in such a way that, we can efficiently answer the query to the dynamic graphs. In~\cite{LB+15}, the authors addressed scalability and efficiency in terms of storage of dynamically evolving graphs by taking advantages of the commonalities of the graph at different time points of the evolution. However, the techniques are not related to our work because, none of these works discuss about dense structure enumeration problem.}
}
\remove{
Our work differs from these in that we aim for {\em change-sensitive} algorithms whose cost is proportional to the magnitude of the change. Prior algorithms on maximal clique maintenance in a dynamic graph  have not been shown to be change-sensitive. Further, prior work has not considered the magnitude of change in the set of maximal cliques in a dynamic graph.
}

\textbf{Roadmap:} We present preliminaries in Section~\ref{sec:prelim}, followed by algorithms for enumerating the change in Section~\ref{sec:csalgo}, magnitude of change in Section~\ref{sec:sizeofchange}, and experimental results in Section~\ref{sec:expts}.


==> size_of_change.tex.bak.tex <==
%------------------------------------------------------------
%\section{Size of $\Lambda(G,G+H)$}
\section{Magnitude of Change}
\label{sec:sizeofchange}
\newcommand{\eps}{\varepsilon}
%----------------------------------------

\remove{
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%--------------------------------------------------
\subsection{Addition of a Single Edge}
%--------------------------------------------------
In the case when a single edge is added to graph $G$, we show the following exact expression for the size of $\Lambda(G,G+e)$.

%------------------
\begin{lemma}
\label{th1}
For an integer $n > 2$, graph $G$ with $n$ vertices, and any edge $e \notin E(G)$, the maximum size of $\Lambda(G,G+e)$ is $3f(n-2)$, and for each $n$, there exists a graph $G$ and edge $e$ that achieve this bound.
\end{lemma}
%------------------

The proof of this Lemma has two parts. Lemma~\ref{l6} shows that the size of $\Lambda(G,G+e)$ can be as large as $3f(n-2)$ and Lemma~\ref{l5} shows that the size of $\Lambda(G,G+e)$ can be no more than $3f(n-2)$.

%------------------
\begin{lemma}
\label{l6}
For any integer $n > 2$ there exists a graph $G$ on $n$ vertices and an edge $e \notin E(G)$ such that $|\Lambda(G,G+e)| = 3f(n-2)$.
\end{lemma}
%------------------

%------------------
\begin{proof}

We use proof by construction. $G$ is a graph on vertex set $\{1,2,\ldots,n\}$. Let $V' = \{1,2,\ldots,n-2\}$. We add edges among vertices of $V'$ such that $G'$, the induced subgraph on vertex set $V'$, becomes a Moon-Moser graph on $(n-2)$ vertices, using the construction in~\cite{MM65}. In addition, we add an edge from every vertex in $V'$ to every vertex in $\{n-1, n\}$. We add edge $e=(n-1,n)$ to $G$ to get graph $G+e$. We claim that the size of $\Lambda(G,G+e)$ is $3f(n-2)$.

%{\bf Picture here.}\\
First, we note that the total number of maximal cliques in $G$ is $2f(n-2)$. Each maximal clique in $G$ contains either vertex $n-1$ or $n$, but not both. The number of maximal cliques in $G$ that contain vertex $n-1$ is $f(n-2)$, since each maximal clique in $G'$ leads to a maximal clique in $G$ by adding $n-1$. Similarly, the number of maximal cliques in $G$ that contain vertex $n$ is $f(n-2)$, leading to a total of $2f(n-2)$ maximal cliques in $G$.

Next, we note that the total number of maximal cliques in $G+e$ is $f(n-2)$. To see this, note that each maximal clique in $G+e$ contains both vertices $n-1$ and $n$, since they can always extend any clique that does not contain them. Further, for each maximal clique in $G'$ we get a corresponding maximal clique in $G+e$ by adding vertices $n-1$ and $n$. Hence, the number of maximal cliques in $G+e$ equals the number of maximal cliques in $G'$, which is $f(n-2)$.

No maximal clique in $G$ can contain both $n-1$ and $n$, while every maximal clique in $G+e$ contains both $n-1$ and $n$. Hence, we have that $\cliques(G)$ and  $\cliques(G+e)$ are disjoint sets, and $\Lambda(G,G+e) = |\cliques(G)| + |\cliques(G+e)| = 3f(n-2)$.
\end{proof}
%------------------

Before proving the other direction (Lemma~\ref{l5}), we need the following results.  

\begin{lemma}
\label{l1234}
For a graph $G$:
\begin{itemize}
\itemsep0em 
	\item[(a)]
		For any $v\in V(G)$, $|\cliques_{v}(G)| \leq f(n-1)$.
	\item[(b)]
		For any $e\in E(G)$, the number of maximal cliques in $G$ containing $e$ is at most $f(n-2)$.
	\item[(c)]
		For any edge $e \notin E(G)$, any clique in $\cliques(G+e) \setminus \cliques(G)$ must contain $e$.
	\item[(d)]
		For any edge $e = (u,v) \notin E(G)$, any clique in $\cliques(G) \setminus \cliques(G+e)$ must contain either $u$ or $v$.
\end{itemize}
\end{lemma}

\begin{proof}
\begin{itemize}
\itemsep0em
	\item[(a)]
		Each maximal clique $c$ in $G$ that contains $v$ corresponds to a unique maximal clique in graph $G-v$ that can be derived by deleting vertex $v$ from $c$. Thus, the  number of maximal cliques in $G$ that contain $v$ can be no more than the maximum number of maximal cliques in $G-v$, which is $f(n-1)$.
	\item[(b)]
		Consider any edge $(u,v) \in E(G)$. Let vertex set $V' = \left( \Gamma_G(u) \cap \Gamma_G(v) \right) -\{u,v\}$, and let $G'$ be the subgraph of $G$ induced by $V'$. Each maximal clique in $G$ that contains edge $(u,v)$ corresponds to a unique maximal clique in $G'$, by simply deleting vertices $u$ and $v$. And each maximal clique in $G'$ corresponds to a unique maximal clique in $G$ that contains $(u,v)$ by adding vertices $u$ and $v$. Hence, there is a bijection between the maximal cliques in $G'$ and the set of maximal cliques in $G$ that contain $(u,v)$. The number of maximal cliques in $G'$ can be at most $f(n-2)$ since $G'$ has no more than $(n-2)$ vertices.
	\item[(c)]
		Proof by contradiction. Suppose there is a clique $c$ in $\cliques(G+e) - \cliques(G)$ that does not contain $e$. Then, $c$ must be present in $G$ but is not maximal in $G$, and there must be another vertex $v \in V(G)$ that can be added to $c$ while remaining a clique. Clearly, $v$ can be added to clique $c$ in $G + e$ also, so that $c$ is not maximal in $G + e$, contradicting our assumption.
	\item[(d)]
		Proof by contradiction. Suppose there is a maximal clique $c$ in $\cliques(G) - \cliques(G +e)$ that contains neither $u$ nor $v$. Then, $c$ must be a maximal clique in $G$. Since $c$ is not a maximal clique in $G + e$, $c$ is a proper subset of another maximal clique $c'$ in $\cliques(G+ e)$. From Lemma~\ref{l1234}(c), $c'$ must contain edge $e = (u,v)$, and hence, both vertices $u$ and $v$.  Since $c'$ is a clique, every vertex in $c'$ is connected to $u$, even in $G$. Hence, every vertex in $c$ is connected to $u$ even in $G$. Therefore $c \cup \{u\}$ is a clique in $G$, and $c$ is not maximal in $G$, contradicting our assumption. 
\end{itemize}
\end{proof}

%--------------------
\begin{lemma}
\label{l5}
For a graph $G$ on $n$ vertices and edge $e \notin E(G)$, the size of $\Lambda(G,G+e)$ can be no larger than $3f(n-2)$.
\end{lemma}
%--------------------

%--------------------
\begin{proof}
Proof by contradiction. Suppose there exists a graph $G$ and edge $e\notin E(G)$ such that $|\Lambda(G,G+e)| > 3f(n-2)$. Then either $|\cliques(G+e) \setminus \cliques(G)| > f(n-2)$ or $|\cliques(G) \setminus \cliques(G+e)| > 2f(n-2)$.\\

\textbf{Case 1:} $|\cliques(G+ e) \setminus \cliques(G)| > f(n-2)$: This means that total number of new maximal cliques formed due to addition of edge $e$ is larger than $f(n-2)$. From Lemma~\ref{l1234} it follows that,
\begin{itemize}
\itemsep0em 
	\item Each new maximal clique formed due to addition of edge $e$ must contain $e$.
	\item The total number of maximal cliques in an $n$ vertex graph containing a specific edge can be at most $f(n-2)$.
\end{itemize}

Thus, the number of new maximal cliques after adding edge $e$ is at most $f(n-2)$, contradicting our assumption.\\

\textbf{Case 2:} $|\cliques(G) \setminus \cliques(G+e)| > 2f(n-2)$: Using Lemma~\ref{l1234}(d), each maximal clique $c \in \cliques(G) \setminus \cliques(G+e)$ must contain either $u$ or $v$, but not both. Suppose that $c$ contains $u$ but not $v$. Then $c$ must be a maximal clique in $G-v$. Using Lemma~\ref{l1234}(a), we see that the number of maximal cliques in $G-v$ that contain a specific vertex $u$ can be no more than $f(n-2)$; hence the number of possible cliques $c$ that contain $u$ is no more than $f(n-2)$.  In a similar way, the number of possible maximal cliques that contain $v$ is at most $f(n-2)$. Therefore, the total number of maximal cliques in $\cliques(G) \setminus \cliques(G+e)$ is at most $2f(n-2)$, contradicting our assumption.
\end{proof}
%------------
}
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------

\subsection{Maximum Possible Change in the Set of Maximal Cliques}
 
We first consider the maximum change in the set of maximal cliques upon the addition of edges to the graph. For an integer $n$, let $\lambda(n)$ be the maximum size of $\Lambda(G,G+H)$ taken over all possible $n$ vertex graphs $G$ and edge sets $H$. We present the following result with nearly tight bounds on the value of $\lambda(n)$.

%------------
\begin{theorem}
\label{thm:lambdan}
\begin{eqnarray*}
\frac{16}{9}f(n) \le & \lambda(n) & < 2f(n) \qquad \mbox{~if~ $(n \mod 3) = 0$} \\
                             & \lambda(n) & = 2f(n)  \qquad \mbox{~if~ $(n \mod 3) = 1$} \\
\frac{11}{6}f(n) \le & \lambda(n) & < 2f(n) \qquad \mbox{~if~ $(n \mod 3) = 2$} \\
\end{eqnarray*}
\end{theorem}
%------------

\begin{proof}

We first note that $\lambda(n) \le 2f(n)$ for any integer $n$. To see this, note that for any graph $G$ on $n$ vertices and edge set $H$, it must be true from Theorem~\ref{thm:MM65} that $|\cliques(G)| \le f(n)$ and $|\cliques(G+H)| \le f(n)$. Since $|\Lambda^{new}(G,G+H)| \le |\cliques(G+H)|$ and $|\Lambda^{del}(G,G+H)| \le |\cliques(G)|$, we have $|\Lambda(G,G+H)| = |\Lambda^{new}(G,G+H)| + |\Lambda^{del}(G,G+H)| \le |\cliques(G)| + |\cliques(G+H)| \le 2f(n)$.

The result of Moon and Moser~\cite{MM65} states that for $n \ge 2$, there is only one graph $H_n$ on $n$ vertices (subject to isomorphism) that has $f(n)$ maximal cliques. We show below that there is an error in this result for the case $(n \mod 3) = 1$. Note that the result is still true in the cases $(n \mod 3)$ equals $0$ or $2$. Thus for the cases where $(n \mod 3)$ is $0$ or $2$, adding or deleting edges from $H_n$ leads to a graph with fewer than $f(n)$ maximal cliques, so that we can never achieve a change of $2f(n)$ maximal cliques. Thus we have that for $(n \mod 3)$ equal to $0$ or $2$, $\lambda(n)$ is strictly less than $2f(n)$. The case of $(n \mod 3) = 1$ is discussed separately (see Observation~\ref{obs:mm} below).


We next show that there exists a graph $G$ on $n$ vertices and an edge set $H$ such that the size of $\Lambda(G,G+H)$ is large. See Figure~\ref{fig:size-of-change} for an example. Graph $G$ is constructed on $n$ vertices as follows. Let $\eps > 3$ be an integer. Choose $\eps$ vertices in $V(G)$ into set $V_1$. Let $V_2 = V \setminus V_1$. Edges of $G$ are constructed as follows. 
\begin{itemize}
\itemsep0em 
\item
Each vertex in $V_1$ is connected to each vertex in $V_2$.
\item
Edges are added among vertices of $V_2$ to make the induced subgraph on $V_2$ a Moon-Moser graph on $(n-\eps)$ vertices. Let $G_2$ denote this induced subgraph on $V_2$, which has $f(n-\eps)$ maximal cliques.
\item 
There are no edges among vertices of $V_1$ in $G$.
\end{itemize}

It is clear that for each maximal clique $c$ in $G_2$ and vertex $v \in V_1$, there is a maximal clique in $G$ by adding $v$ to $c$. Thus the number of maximal cliques in $G$ is $|V_1| \cdot |\cliques(G_2)|$. Hence we have 
\begin{equation}
\label{eqn:1}
|\cliques(G)|  = \eps \cdot f(n-\eps)
\end{equation}

To graph $G$, we add the edge set $H$, constructed as follows. $H$ consists of edges connecting vertices in $V_1$, to form a Moon-Moser graph on $\eps$ vertices. Let $G' = G + H$. We note that $\cliques(G)$ and $\cliques(G')$ are disjoint sets. To see this, note that each maximal clique in $G$ contains exactly one vertex from $V_1$, since no two vertices in $V_1$ are connected to each other in $G$. On the other hand, each maximal clique in $G'$ contains more than one vertex from $V_1$, since each vertex $v \in V_1$ is connected to at least one other vertex in $V_1$ in $G'$. Hence, $\Lambda(G,G') = \cliques(G) \cup \cliques(G')$, and
\begin{equation}
\label{eqn:2}
|\Lambda(G,G')| = |\cliques(G)| + |\cliques(G')|
\end{equation}

To compute $|\cliques(G')|$, note that since each vertex in $V_1$ is connected to each vertex in $V_2$, for each maximal clique in $G'(V_1)$ and each maximal clique in $G'(V_2)$, we have a unique maximal clique in $G'$. There are $f(\eps)$ maximal cliques in $G'(V_1)$ and $f(n-\eps)$ maximal cliques in $G'(V_2)$, and hence we have
\begin{equation}
\label{eqn:3}
|\cliques(G')| = f(\eps) \cdot f(n-\eps)
\end{equation}

Putting together Equations~\ref{eqn:1},~\ref{eqn:2}, and~\ref{eqn:3} we get 

\begin{equation}
\label{eqn:4}
|\Lambda(G,G')| = (\eps + f(\eps)) \cdot f(n-\eps)
\end{equation}

Let $F(\eps) = (\eps + f(\eps))f(n-\eps)$. We compute the value of $\eps (> 3)$ at which $F(\eps)$ is maximized. To do this, we consider three different cases depending on the value of $(n \mod 3)$, and omit the calculations. If $n\mod 3 = 0$, $F(\eps)$ is maximized at $\eps = 4$ and the maximum value $F(4) = \frac{16}{9}f(n)$. If $n\mod 3 = 1$, $F(\eps)$ is maximized at $\eps = 4$ and $F(4) = 2f(n)$. And finally if $n\mod 3 = 2$, $F(\eps)$ is maximized at $\eps= 5$ and $F(5) = \frac{11}{6}f(n)$. This completes the proof.
\end{proof}
%------------------------------------------------------------------------------

%-------------------------------------------------------------------------------------
\begin{figure*}
\centering
\begin{tabular}{c}
	%\hspace{-2mm}
	\includegraphics[width=.5\textwidth]{pic2.png}\\
\end{tabular}
\caption{\textbf{Construction showing a large change in set of maximal cliques when a few edges are added. On the left is $G$, the original graph with $n$ vertices where each vertex in $V_1$ is connected to each vertex in $V_2$, and $V_1$ is an independent set. In $G$, the induced subgraph $G_2$ on vertex set $V_2$ forms a {\tt Moon-Moser} graph. On the right is $G'$, the graph formed after adding edge set $H$ to $G$ such that the induced subgraph on vertex set $V_1$ becomes a {\tt Moon-Moser} graph. Let $c$ be a clique in $G_2$, and $c'$ a new clique in $G'$ formed among vertices in $V_1$. Note that $c\cup\{v\}$ was a maximal clique in $G$, and is now subsumed by a new maximal clique $c\cup c'$.}}
\label{fig:size-of-change}
%fig7
\end{figure*}
%-------------------------------------------------------------------------------------


%for arxiv
%------------------------------------------------------------------------------
\begin{figure*}
\centering
\begin{tabular}{c}
\includegraphics[width=.5\textwidth]{moon_moser.png}\\
\end{tabular}
\caption{\textbf{For the case $(n \mod 3) = 1$, $H_n$ and $G_n$ are non-isomorphic graphs on $n$ vertices, with $f(n)$ maximal cliques each, showing a counterexample to Theorem 2 of Moon and Moser~\protect\cite{MM65}.}}
\label{fig:moon-moser}
\end{figure*}
%------------------------------------------------------------------------------

\subsection{An Error in a Result of Moon and Moser (1965)}
Moon and Moser~\cite{MM65}, in Theorem 2 in their paper, claim ``For any $n \ge 2$, if a graph $G$ has $n$ nodes and $f(n)$ cliques, then $G$ must be equal to $H_n$", where $H_n$ is a specific graph, described below. We found that this theorem is incorrect for the case when $(n \mod 3) = 1$.

The error is as follows (see Figure~\ref{fig:moon-moser}). For $(n \mod 3) = 1$, the graph $H_n$ is constructed on vertex set $V_n=\{1,2,\ldots,n\}$ by taking vertices $\{1,2,3,4\}$ into a set $S_0$ and dividing the remaining vertices into groups of three, as sets $S_1,S_2,\ldots,S_{\frac{n-4}{3}}$. In graph $H_n$, edges are added between any two vertices $u,v$ such that $u \in S_i$, $v \in S_j$ and $i \neq j$. This graph $H_n$ has $4\cdot 3^{\frac{n-4}{3}}$ maximal cliques, since we can make a maximal clique by choosing a vertex from $S_0$ (4 ways), and one vertex from each $S_i, i > 0$ (3 ways for each such $S_i, i = 1\ldots (n-4)/3$). 

Contradicting Theorem 2 in~\cite{MM65}, we show there is another graph $G_n$ that is different from $H_n$, but still has the same number of maximal cliques. $G_n$ is the same as $H_n$, except that the vertices within $S_0$ are connected by a cycle of length $4$. In this case, we can still construct $4\cdot 3^{\frac{n-4}{3}}$ maximal cliques, since we can make a maximal clique by choosing two connected vertices in $S_0$ (4 ways to do this), and one vertex from each $S_i, i > 0$ (3 ways for each such $S_i, i = 1\ldots (n-4)/3$).

%--------------------------------------------------
\begin{observation}
\label{obs:mm}
For the case $(n \mod 3) = 1$, there are two distinct non-isomorphic graphs $H_n$ and $G_n$  described above, that have $4\cdot 3^{\frac{n-4}{3}}$ maximal cliques, which is the maximum possible. This is a correction to Theorem 2 of Moon and Moser~\cite{MM65}, which states that there is only one such graph, $H_n$.
\end{observation}
%--------------------------------------------------

This observation enables us to have $\lambda(n) = 2f(n)$ for the case $(n \mod 3) = 1$. By starting with graph $H_n$ and by adding edges to make it $G_n$, we remove $f(n)$ maximal cliques and introduce $f(n)$ maximal cliques, leading to a total change of $2f(n)$.

\remove{
%----------------------------------------------------------------------
\subsection{Bound on the size of change parameterized by max degree $\Delta$ of $G$}
%----------------------------------------------------------------------

\begin{lemma}
For any $v\in V(G)$, $|\cliques_{v}(G)| \leq f(\Delta)$ where $\Delta$ is the maximum degree of $G$.
\end{lemma}

\begin{proof}
Each maximal clique $c$ of $G$ that contains $v$ must be within the neighborhood of $v$ and the size of this neighborhood can be at most $\Delta$. Thus, there can be at most $f(\Delta)$ maximal cliques each of which contains $v$. 
\end{proof}

\begin{lemma}
For any $e\in E(G)$, the number of maximal cliques in $G$ containing $e$ is at most $f(\Delta-1)$.
\end{lemma}

\begin{proof}
Suppose each of the vertices $u$ and $v$ of an edge $e$ has degree $\Delta$ and that $u$ and $v$ has the same neighborhood. Thus the size of the neighborhood except $u$ and $v$ is $\Delta-1$. There can be at most $f(\Delta-1)$ maximal cliques within these vertices. Now when we add $u$ and $v$ to each of such maximal clique, a new maximal clique will be formed that contains the edge $e$. Thus there can be at most $f(\Delta-1)$ such maximal cliques.
\end{proof}

\begin{lemma}
For a graph $G$ on $n$ vertices and edge $e\notin E(G)$, the size of $\Lambda(G,G+e)$ can be no larger than $3f(\Delta)$.
\end{lemma}

\begin{proof}
Proof by contradiction. Suppose there exists  a graph $G$ and edge $e\notin E(G)$ such that $|\Lambda(G,G+e)| > 3f(\Delta)$. Then either $|\cliques(G+e)\setminus\cliques(G)| > f(\Delta)$ or $|\cliques(G)\setminus\cliques(G+e)| > 2f(\Delta)$.

\textbf{Case 1:} $|\cliques(G+e)\setminus\cliques(G)| > f(\Delta)$: This means that the total number of new maximal cliques is more than $f(\Delta)$. Assume that $e = (u,v)$, $U = \Gamma_G(u) = \Gamma_G(v)$, and $|U| = \Delta$. Then there can be at most $f(\Delta)$ maximal cliques in the subgraph of $G$ induced by $U$. For each such maximal clique, there will be a new maximal clique by adding $e$. Thus the number of new maximal cliques is at most $f(\Delta)$. A contradiction.

\textbf{Case 2:} $|\cliques(G)\setminus\cliques(G+e)| > 2f(\Delta)$: First note that each subsumed clique contains either $u$ or $v$ but not the both. Next, the number of maximal cliques in $G$ is at most $f(\Delta)$ containing $u$ and $f(\Delta)$ containing $v$. Thus the total number of subsumed cliques is at most $2f(\Delta)$. A contradiction. 
\end{proof}

\begin{lemma}
For any integer $n > 2$ there exists a graph $G$ on $n$ vertices with maximum degree $\Delta$ and an edge $e\notin E(G)$ such that $|\Lambda(G,G+e)| = 3f(\Delta)$.
\end{lemma}

\begin{proof}
We use proof by construction. Let $G$ be a graph on $n$ vertices and $X$ be a subset of $V(G)$ of size $\Delta$. Also assume that $X$ forms a Moon-Moser graph.Note that degree of every vertex of $X$ is at most $\Delta-1$ within $X$. Fix two vertices $u$ and $v$ and connect from each of $u$ and $v$ to all the vertices of $X$. Connect among rest of the vertices in such a way that the maximum degree in $G$ does not exceed $\Delta$. This completes the construction of $G$.

First note that total number of maximal cliques containing $u$ in $G$ is $f(\Delta)$ and total number of maximal cliques containing $v$ in $G$ is $f(\Delta)$. This is because, each maximal clique in $X$ will be maximal in $G$ when adding $u$ and when adding $v$. Total number of such maximal cliques is thus $2f(\Delta)$ that contains either $u$ or $v$ but not both.

Next note that total number of maximal cliques in $G+e$ containing $e = (u,v)$ is $f(\Delta)$. This is because, each maximal clique in $X$ becomes a new maximal clique in $G+e$ when $e$ is added and these are all inclusive new maximal cliques because, neither $u$ nor $v$ is connected to any other vertex in $G$ except $X$. Also note that each maximal clique in $G$ containing either $u$ or $v$ will becomes part of a new maximal clique and thus will be subsumed.

Thus, $|\Lambda(G,G+e)| = |\cliques_u(G)| + |\cliques_v(G)| + f(\Delta) = 3f(\Delta)$. 
\end{proof}
}

\remove{
%----------------------------------------------------------------------
\subsection{Bound on the size of change parameterized by degeneracy $d$ of $G$}
%----------------------------------------------------------------------
Graph degeneracy is a measure of graph sparsity. Degeneracy is the smallest value $d$ such that every subgraph of $G$ has at least a vertex of degree at most $d$. In other words, it is the maximum over minimum degrees of all the subgraphs of $G$. When the degeneracy $d$ is known, the maximum number of maximal cliques of $d$-degenerate graph is different from the moon-moser bound as shown in~\cite{ELS10}. First we prove a lower bound on $|\Lambda(G,G+e)|$ as follows:

\begin{lemma}
For any integer $n > 2$, there exists a graph $G$ with $n$ vertices and degeneracy $d$ such that $|\Lambda(G,G+e)|$  is at least $3(n-d)f(d-2)$ where $e\notin E(G)$.
\end{lemma}

\begin{proof}
We prove by construction. Suppose there is a graph $G$ with $n$ vertices and $V = \{1, 2, 3, ..., n-1, n\}$. Now assume that first $n-d$ vertices (denote as set $A$) form an independent set, followed by next $(d-2)$ vertices (denote as set $B$) that forms a moon-moser graph, followed by vertices $n-1$ and $n$ that are not connected but each is connected to the rest $n-1$ vertices. Each vertex in set $A$ is connected to each vertex in set $B$. Clearly, the degeneracy of $G$ is $d$. Now there are $(n-d)f(d-2)$ maximal cliques in $G' = G-\{n-1,n\}$ and assume $\cliques(G')$ denotes the set of maximal cliques in $G'$. For each clique $c'$ in $\cliques(G')$, we get two maximal cliques in $G$, once by adding $n-1$ to $c'$ and then by adding $n$ to $c'$. Thus, $|\cliques(G)| = 2(n-d)f(d-2)$. When we add an edge $e$ between $n-1$ and $n$ each clique in $\cliques(G')$ is extended by both $n-1$ and $n$ and becomes a maximal clique in $G+e$. Note that $\cliques(G)$ and $\cliques(G+e)$ are disjoint set. To see this, observe that each maximal clique in $G$ contains either $n-1$ or $n$ since $n-1$ and $n$ are not connected in $G$. On the other hand, each maximal clique in $G+e$ contains both $n-1$ and $n$ and $|\cliques(G+e)| = |\cliques(G')| = (n-d)f(d-2)$. Hence, $\Lambda(G,G+e) = \cliques(G)\cup\cliques(G+e)$ and $|\Lambda(G,G+e)| = |\cliques(G)| + |\cliques(G+e)| = 3(n-d)f(d-2)$.
\end{proof}


Next, we will prove an upper bound on $|\Lambda(G,G+e)|$ in Lemma~\ref{upper_bound}. For proving an upper bound, we use the following results and some supporting lemmas in obtaining bound on the size of change in our case:

\begin{lemma}[Theorem 3 of~\cite{ELS10}]
Let $d$ be a multiple of $3$ and $n \geq d+3$. Then the largest possible number of maximal cliques in an n-vertex graph with degeneracy $d$ is $(n-d)3^{\frac{d}{3}}$.
\end{lemma}

This result assumes that $d$ is multiple of $3$. However, we can generalize the bound that works for any  value of the degeneracy $d$ as follows:

\begin{lemma}\label{degen:1}
Let $d$ be the degeneracy of an $n$ vertex graph $G$. Then maximum number of maximal cliques in $G$ is $(n-d)f(d)$. 
\end{lemma}
\begin{proof}
\textbf{Upper Bound: } We will show that number of maximal cliques in a graph $G$ with $n$ vertices and degeneracy $d$ is no more than $(n-d)f(d)$. For this, assume that there is a degeneracy ordering of the vertices of $G$ for which there are at most $d$ neighbors of each vertex that come later in the ordering. Consider first $(n-d)$ vertices in this ordering and denote this set of vertices as $S$. Now, each vertex in $S$ is connected to at most $d$ vertices in set $V\setminus S$. Also, there are precisely $d$ vertices in the set $S' = V\setminus S$. Now, the maximum possible number of maximal cliques formed using the vertices in $S'$ is $f(d)$. As each vertex in $S$ is connected to at most $d$ vertices in $S'$, each such vertex can participate in at most $f(d)$ maximal cliques. Thus, maximum number of maximal cliques in $G$ is $(n-d)f(d)$. 

\textbf{Lower Bound: } Next we will show that there exists a graph $G$ with $n$ vertices and degeneracy $d$ such that there are $(n-d)f(d)$ maximal clique. We will show this using a construction. Assume that vertices in $S'$ forms a moon-moser graph. Next, the vertex set $S$ is an independent set and each vertex in $S$ is connected to all vertices in $S'$. This completes the construction of $G$. Note that, number of maximal cliques in the induced subgraph with vertex subset $S'$ is $f(d)$. Each maximal clique in that subgraph together with each vertex in $S$ forms a distinct maximal clique in $G$. Thus, total number of maximal clique in $G$ is $|S|f(d)$ which is $(n-d)f(d)$. This completes the proof. 
\end{proof}

\begin{lemma}\label{degen:2}
For any $v\in V(G)$, $|\cliques_v(G)| \leq (n-d-1)f(d)$ where $d$ is the degeneracy of the graph $G$
\end{lemma}

\begin{proof}
Suppose there is a vertex $v$ such that $v$ is connected to $n-1$ vertices. Also, assume that the degeneracy of $G$ is $d$. Now, the degeneracy of $G-v$ can be at most $d$. Now, the maximum number of maximal cliques in $G-v$ is $(n-d-1)f(d)$. Each of these maximal clique when includes $v$ becomes a maximal clique in $G$. Thus maximum number of maximal cliques containing a vertex is at most $(n-d-1)f(d)$.
\end{proof}

\begin{lemma}\label{degen:3}
For any $e\in E(G)$, the number of maximal cliques containing $e$ is at most $(n-d-2)f(d)$ where $d$ is the degeneracy of $G$.
\end{lemma}

\begin{proof}
Suppose that $e = (u,v)$ and each of $u$ and $v$ is connected to rest of the vertices of $G$. Also the degeneracy of $G-u-v$ can be at most $d$. Now, the maximum number of maximal cliques in $G-u-v$ is $(n-d-2)f(d)$. Each of these maximal cliques, when includes $u$ and $v$, becomes a maximal cliques in $G$. Thus, maximum number of maximal cliques containing $e$ is $(n-d-2)f(d)$.
\end{proof}

\begin{lemma}\label{upper_bound}
For a graph $G$ on $n$ vertices and edge $e\notin E(G)$, the size of $\Lambda(G,G+e)$ can be no larger than $3(n-d-2)f(d)$ where $d$ is the degeneracy of the graph $G$.
\end{lemma}


\begin{proof}
Proof by contradiction. Suppose there exists a graph $G$ and an edge $e\notin E(G)$ such that $|\Lambda(G,G+e)| > 3(n-d-2)f(d)$. Then, either $|\cliques(G+e)\setminus\cliques(G)| > (n-d-2)f(d)$ or $|\cliques(G)\setminus\cliques(G+e)| > 2(n-d-2)f(d)$.
\end{proof}

\begin{proof}
\textbf{Case 1: }$|\cliques(G+e)\setminus\cliques(G)| > (n-d-2)f(d):$ Assume that $e = (u,v)$ and each of $u$ and $v$ are connected to the rest $n-2$ vertices of $G$. Note that the degeneracy of $G-u-v$ is at most $d$. So, maximum number of maximal cliques in $G-u-v$ is $(n-d-2)f(d)$. When we add $e$, each maximal clique in $G-u-v$ together with $u$ and $v$ becomes a maximal clique in $G$ and each of these maximal clique contains $e$. Thus $|\cliques(G+e)\setminus\cliques(G)| \leq (n-d-2)f(d)$. A contradiction.

\textbf{Case2: }$|\cliques(G)\setminus\cliques(G+e)| > 2(n-d-2)f(d):$ Using Lemma~\ref{l1234}(d), each maximal clique $c \in \cliques(G) \setminus \cliques(G+e)$ must contain either $u$ or $v$, but not both. Suppose that $c$ contains $u$ but not $v$. Then $c$ must be maximum clique in $G-v$. Using Lemma~\ref{degen:2} we see that the number of maximal cliques in $G-v$ that contains a specific vertex $u$ can be no more than $(n-d-2)f(d)$; hence the number of possible maximal cliques that contain $u$ is no more than $(n-d-2)f(d)$. In a similar way, the number of possible maximal cliques that contain $v$ is at most $(n-d-2)f(d)$. Therefore, the total number of maximal cliques in $\cliques(G)\setminus\cliques(G+e)$ is at most $2(n-d-2)f(d)$. This is a contradiction.
\end{proof}

}

